Large Language Models for Requirements Engineering: A Cross-Task Empirical Evaluation

Requirements-related information is scattered across heterogeneous artefacts such as user feedback, developer discussions, and software repositories, making the extraction of actionable requirements knowledge labour-intensive and hard to scale. Large Language Models (LLMs) can support many Requirements Engineering (RE) activities, from classification and traceability identification to specification and explanation generation, but existing evidence is fragmented across tasks, artefact types, and evaluation settings, and studies rarely offer cross-task evaluations or replication packages. We present two complementary empirical studies evaluating LLMs across five RE-related activities. The first is a controlled experiment on five lightweight open-source LLMs for feedback-driven requirements classification and specification generation. The second is an exploratory industrial case study on two frontier LLMs for traceability link identification and traceability explanation generation using real project artefacts. Classification and traceability identification were assessed with quantitative metrics, and generation tasks through human evaluation. LLM performance is strongly task-dependent, ranging from moderate to high, and no single model consistently outperformed the others, indicating that effective adoption depends on selecting models and prompting strategies per task. Our contributions are: (i) the first cross-task empirical evaluation of LLMs spanning five RE-related activities, (ii) replication materials supporting reproducibility, and (iii) a broader understanding of the capabilities, limitations, and practical readiness of current LLMs for RE.

==> study-1/background.tex <==
We now define key terms and formulate the problems of user feedback classification and requirements specification. We also provide a concise illustrative example.

\textbf{Definition 1 (User Feedback).} A user feedback instance is denoted as \( r \), representing a textual message written by a user about an application. 
The set of all feedback messages for an application \( a \) is \( R = \{r_1, r_2, ..., r_n\} \).

This study focuses on app reviews, a form of user feedback from mobile platforms (e.g., Google Play Store). Such feedback conveys diverse information useful for RE; in this work, we particularly focus on user requests and  NFRs.

\noindent\textbf{Definition 2 (User Request).} 
A user request \( t_{UR} \) is an expressed intent in a feedback instance, which can be of a type \textit{feature request}, or \textit{bug report}.

\noindent\textbf{Definition 3 (Non-Functional Requirement).} 
A non-functional requirement \( t_{NFR} \) is a reference in a feedback instance to one of the eight quality attributes of the application (e.g., \textit{usability}) as defined in ISO/IEC 25010~\cite{iso25010}.

Our study addresses two main problems: user feedback classification and requirements specification, as defined below. 

\noindent\textbf{Problem 1 (User Feedback Classification).} 
Given a set of user feedback instances \( R = \{r\} \) for an application \( a \), find a multi-set \( C = \{t\} \), where \( t \) is an information type assigned to a feedback instance \( r \in R \). The type classification is performed either on user-request types \( t_{UR} \) or on NFR types \( t_{NFR} \), each with an additional \textit{other} category to capture feedback outside these types.

\noindent\textbf{Problem 2 (Requirements Specification Generation).} 
Given a set of user feedback instances \( R = \{r\} \) for an application \( a \) and their associated information types \( C = \{t\} \), generate a set of requirement statement \( S = \{s\} \), where each \( s \) is a written statement that formalizes or summarizes the user needs expressed in one or more feedback instances \( r \in R \). 


\JAC{\noindent\textbf{Illustrative Example.}
Let \( R = \{r_1, r_2, r_3\} \) be a set of user feedback instances for an application \( a \),
where \( r_1 \) states ``The app crashes when saving a form'',
\( r_2 \) states ``I want the app to automatically save my progress'',
and \( r_3 \) states ``The app responds very slowly when opening large files''.
According to Problem~1, the resulting multi-set of information types is
\( C = \{t_1, t_2, t_3\} \),
where \( t_1 = \textit{bug report} \), as \( r_1 \) reports incorrect system behavior;
\( t_2 = \textit{feature request} \), as \( r_2 \) explicitly expresses a desired functionality;
and \( t_3 = \textit{performance} \) NFR, as \( r_3 \) refers to system response time.
Following Problem~2, a generated requirements specification in the form of a user story derived from \( r_2 \) is
\( s \):
\textit{``As a user, I want the app to automatically save my progress so that I do not lose data.''}}



==> study-1/conclusion.tex <==
Analysing online user feedback is important for RE tasks, yet automation remains challenging. This study presents the first systematic evaluation of \JAC{open-source}, lightweight LLMs for feedback-driven RE. Five models were evaluated with multiple prompting strategies on three RE tasks: classifying feedback by user request and NFR type, and generating requirement specification.

Lightweight LLMs classified user request types accurately (F1 $\approx$ 0.74) but performed moderately for NFRs (F1 $\approx$ 0.55). Structured prompting improved results slightly. Generated specification was generally complete and coherent but often verbose and sometimes included fabricated requirements. Lightweight LLMs can support early RE activities, but still require human oversight.

We release our evaluation framework and replication package to support further research~\cite{mallya2026from}. Future work should explore fine-tuning lightweight \JAC{open-source} LLMs, developing retrieval-augmented pipelines, and creating domain-adapted benchmarks to improve their accuracy and reliability in RE. \JAC{We also suggest that future studies should empirically benchmark the performance of lightweight LLMs against heavyweight language models (e.g., ChatGPT). This benchmarking would help determine whether the potential performance gains of heavyweight LLMs justify the trade-offs compared to lightweight models.}

==> study-1/scenarios.tex <==
We present three scenarios illustrating how feedback classification and requirements generation support RE, inspired by real cases~\cite{AlSubaihin2021}, and prior studies~\cite{Dabrowski2022}.

\noindent\textbf{Scenario 1 (Supporting Requirements Elicitation).} App reviews often contain implicit requirements expressed as feature requests or bug reports~\cite{Dabrowski2022a}. Understanding these helps product teams capture evolving user needs, identify emerging issues, and plan product improvements. As an example, imagine that after releasing a new version of WhatsApp, the team wants to identify problems users mention in their reviews (e.g., ``messages fail to send'') and desired features (e.g., ``add message scheduling''). Automatically classifying app reviews by request type helps teams quickly identify user needs, while quantifying the feedback shows their user-perceived importance.

\noindent\textbf{Scenario 2 (Supporting Requirements Classification).} Beyond identifying request types, the WhatsApp development team also wants to understand which non-functional qualities users discuss~\cite{Dabrowski2022}. Feedback such as ``too slow to open'' or ``confusing chat layout'' reflects concerns about performance and usability. Automatically classifying feedback by referenced NFRs helps developers identify which quality attributes users value most, revealing whether users are more concerned with performance or usability. This supports task prioritization and helps balance new features with quality improvements.

\noindent\textbf{Scenario 3 (Supporting Requirements Specification).} After identifying and classifying requirements from WhatsApp user feedback, analysts may want to document them clearly and consistently. Translating informal comments into structured requirements is time-consuming and error-prone~\cite{AlSubaihin2021}. For example, feedback such as ``add dark mode'' can be reformulated as ``The system shall provide a dark mode option''. Although such documentation may not produce complete specification, automating it can provide initial drafts that accelerate refinement and maintain traceability with user feedback.

For these scenarios, a tool that classifies user feedback and generates requirements could help the team evolve their app more effectively.


==> study-2/background_2.tex <==
We now introduce the industrial context of the study, defines the key concepts and research problems, and presents the large language models evaluated in our experiments.
	
\subsubsection{Industrial Context}
This study was conducted in the context of the Rust open-source ecosystem. Rust is a general-purpose, cross-platform programming language known for its memory safety guarantees, support for concurrency, and high performance. The language has achieved widespread industrial adoption and is used by organisations such as Huawei, Microsoft, Amazon, and Meta. Rust is developed by a large community of contributors from industry, academia, and the open-source community.

Most Rust development activities take place on GitHub. Contributors use GitHub to manage source code, issues, and pull requests. Technical discussions primarily take place on the Rust Zulip platform. These artefacts contain information about project goals, implementation activities, design decisions, and project progress.

To support planning and coordination, the Rust community introduced the Project Goals initiative. The initiative defines goals for fixed planning cycles. Each goal is documented using a semi-structured template describing its motivation, expected outcomes, and ownership. Accepted goals are linked to GitHub tracking issues that record implementation tasks and progress updates. Dedicated Zulip discussions support coordination and technical decision-making throughout the implementation process.

Information related to a single goal is therefore often distributed across multiple artefacts. A goal may describe the intended outcome, a tracking issue may document implementation progress, and discussions may contain the rationale behind technical decisions. Understanding these relationships often requires contributors to manually inspect multiple sources. This challenge is particularly relevant for industrial stakeholders who need to understand ongoing development activities and their potential impact on products and engineering plans.

The industrial perspective of this study is informed by the authors' involvement in the Rust ecosystem through Huawei's trusted programming initiatives. This study investigates whether large language models can support automated traceability identification and explanation generation across Rust project artefacts.

\subsubsection{Terminology and Problem Formulation}

Requirements-related information in large open-source software projects is distributed across multiple artefacts. Project goals describe planned objectives and expected outcomes. Tracking issues record activities related to achieving these goals. Developer discussions document technical reasoning, implementation decisions, coordination activities, and project progress. Together, these artefacts capture how project objectives are planned, implemented, and discussed over time.

\noindent\textbf{Definition 1 (Goal Artifact).}
A goal artifact is denoted as \( g \), representing a planned project objective or technical initiative. It typically contains motivation, expected outcomes, ownership information, and high-level implementation plans. The set of goal artifacts is denoted as \( G = \{g_1, g_2, ..., g_n\} \).

\noindent\textbf{Definition 2 (Tracking Issue).}
A tracking issue is denoted as \( i \), representing activities related to the implementation of a goal artifact. It may contain task lists, milestones, dependencies, status updates, and progress reports. The set of tracking issues is denoted as \( I = \{i_1, i_2, ..., i_m\} \).

\noindent\textbf{Definition 3 (Discussion Fragment).}
A discussion fragment is denoted as \( d \), representing a textual unit extracted from developer discussions. It may contain implementation details, technical reasoning, design decisions, coordination activities, progress updates, or problem-solving discussions. The set of discussion fragments is denoted as \( D = \{d_1, d_2, ..., d_k\} \).

\noindent\textbf{Definition 4 (Traceability Link).}
A traceability link is denoted as \( l \), representing a relationship between a source artefact and a discussion fragment. The linked artefacts refer to the same project objective, implementation activity, technical decision, dependency, coordination activity, or development effort.

Our study addresses two main problems: traceability identification and explanation generation, as defined below.

\noindent\textbf{Problem 1 (Traceability Identification).}
Given a source artefact \( a \), where \( a \in G \cup I \), and a set of discussion fragments \( D = \{d\} \), find a ranked set of candidate traceability links \( L = \{l\} \), where each \( l \) associates the source artefact with a discussion fragment that is semantically related to the same project objective, implementation activity, technical decision, or development effort.

\noindent\textbf{Problem 2 (Explanation Generation).}
Given a traceability link \( l \) between a source artefact \( a \) and a discussion fragment \( d \), generate an explanation \( e \) describing why the linked artefacts are related. The explanation should include supporting evidence extracted from the artefacts.

\noindent\textbf{Illustrative Example.}
Let \( g \in G \) be a goal artifact describing a planned improvement to the Rust compiler, and let \( i \in I \) be a tracking issue containing implementation tasks required to achieve this goal. Assume a set of discussion fragments \( D = \{d_1, d_2, d_3\} \), where \( d_1 \) discusses implementation details, \( d_2 \) contains design decisions, and \( d_3 \) reports development progress. According to Problem~1, the objective is to identify the discussion fragments most closely related to \( g \) or \( i \), resulting in a ranked set of traceability links \( L \). Following Problem~2, for a selected link \( l = (g, d_2) \), the generated explanation \( e \) should describe that both artefacts discuss the same compiler improvement and provide evidence from the goal description and the developer discussion supporting this relationship.

==> study-2/scenarios-2.tex <==
We present three scenarios that illustrate challenges in understanding and managing requirements-related information in large open-source software projects.

\noindent\textbf{Scenario 1 (Supporting Contributor Onboarding).} New contributors often need to understand why a project goal was introduced and how it relates to ongoing implementation activities. Relevant information is typically distributed across project goals, tracking issues, and developer discussions. Navigating these artefacts manually can be time-consuming and may lead to important information being overlooked. This challenge becomes particularly difficult in large projects where decisions and rationale accumulate over long periods of time.

\noindent\textbf{Scenario 2 (Understanding Goal Evolution).} Project maintainers need to understand how project goals evolve over time and whether ongoing activities support the intended outcomes. While goals describe planned objectives, evidence of their implementation, refinement, and discussion is often scattered across multiple artefacts. Understanding how goals are discussed, modified, and realised therefore requires contributors to examine issues and discussions that may span several months.

\noindent\textbf{Scenario 3 (Supporting Impact Analysis and Planning).} Industrial stakeholders must understand how planned project changes may affect system requirements, dependencies, and development plans. This requires understanding not only project goals but also the discussions and decisions that shape their implementation. Because this information is distributed across multiple artefacts and communication channels, assessing the potential impact of planned changes often requires substantial manual effort and project-specific knowledge.

These scenarios illustrate the challenge of understanding requirements-related information distributed across multiple project artefacts. Automated traceability identification and explanation generation could support understanding of goal implementation, evolution, and rationale.

